SIDM Concerto: Compilation and Data Release of Self-interacting Dark Matter Zoom-in Simulations

We present SIDM Concerto: $14$ cosmological zoom-in simulations in cold dark matter (CDM) and self-interacting dark matter (SIDM) models based on the Symphony and Milky Way-est suites. SIDM Concerto includes one Large Magellanic Cloud- (LMC-) mass system (host mass $\sim 10^{11}~M_{\mathrm{\odot}}$), two Milky Way (MW) analogs ($\sim 10^{12}~M_{\mathrm{\odot}}$), two group-mass hosts ($\sim 10^{13}~M_{\mathrm{\odot}}$), and one low-mass cluster ($\sim 10^{14}~M_{\mathrm{\odot}}$). Each host contains $\approx 2\times 10^7$ particles and is run in CDM and one or more strong, velocity-dependent SIDM models. Our analysis of SIDM (sub)halo populations over seven subhalo mass decades reveals that (1) the fraction of core-collapsed isolated halos and subhalos peaks at a maximum circular velocity corresponding to the transition of the SIDM cross section from a $v^{-4}$ to $v^0$ scaling; (2) SIDM subhalo mass functions are suppressed by $\approx 50\%$ relative to CDM in LMC, MW, and group-mass hosts but are consistent with CDM in the low-mass cluster host; (3) subhalos' inner density profile slopes, which are more diverse in SIDM than in CDM, are sensitive to both the amplitude and shape of the SIDM cross section. Our simulations provide a benchmark for testing SIDM predictions with astrophysical observations of field and satellite galaxies, strong lensing systems, and stellar streams. Data products are publicly available at https://doi.org/10.5281/zenodo.14933624.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

